Search for Optimal Systolic Arrays: A Comprehensive Automated Exploration Framework and Lessons Learned

Systolic arrays have been widely used for accelerating HPC and deep learning applications. There is a plethora of previous works on the performance tuning of systolic arrays, but usually based on a number of oversimplified assumptions (e.g., only considering divisors for loop tiling, pruning based on off-chip data communication) to reduce the design space. In this paper, we present a comprehensive design space exploration tool named Odyssey for systolic array optimization. Odyssey does not rely on artificial assumptions to limit the design space, and yet it is highly efficient and scalable with a hybrid optimization technique. For example, for a 1024x1024x1024 matrix multiplication, it finds designs that reach 90% of the optimal performance in 5 seconds with a single CPU thread. Moreover, using Odyssey, we unveil and quantify the suboptimality introduced by multiple commonly used oversimplifications in prior studies for systolic array design space exploration. For example, Odyssey results show that limiting to divisors for loop tiling leads to a 39% performance loss, and pruning based on off-chip data movement results in a 45% performance loss. We applied Odyssey to explore the architecture trade-offs for matrix multiplication and convolutional neural network, providing inspiration into possible optimizations for these two applications.

==> tex/scope.tex <==
\section{Scope of Odyssey Framework}
\label{sec:scope}
%\todo{[3-3.5, 0.5page]/11}
%This section clarifies the scope of the design space covered by Odyssey and the supported applications.
\subsection{Design Space}
%As introduced in Sections\todo{...}, AutoSA separates the construction of PE arrays and the I/O networks into two stages, computation management and communication management. In each stage, multiple passes of hardware optimizations are applied to boost the compute and communication efficiency of the generated design. AutoSA implements tunable knobs to control each step during the compilation process. Table\todo{...} summarizes the available tuning options in AutoSA.

\begin{table}[t]
\centering
\caption{Scope of AutoSA Design Space Explored by Odyssey.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccccc}
\toprule
\begin{tabular}[c]{@{}c@{}}AutoSA \\ Compilation Pass\end{tabular} &             & \begin{tabular}[c]{@{}c@{}}Space-Time \\ Transformation\end{tabular} & \begin{tabular}[c]{@{}c@{}}Array \\ Partitioning\end{tabular} & \begin{tabular}[c]{@{}c@{}}Latency \\ Hiding\end{tabular} & \begin{tabular}[c]{@{}c@{}}SIMD \\ Vectorization\end{tabular} \\ \toprule
Dataflow  &     & \checkmark    &       &     &    \\ \hline
\multirow{2}{*}{Loop Tiling}    & Divisor     &   & \checkmark  & \checkmark  & \checkmark     \\ \cline{2-6} 
                                & Non-Divisor &   & \checkmark  &             & \\ \hline
Loop Permutation                &             &   & \checkmark  &             &  \\ \bottomrule
\end{tabular}
}
\label{table:odyssey_design_space}
\end{table}

%In this work, we focus on the tuning space of the computation management in AutoSA. We left the communication optimization to be handled by the compiler automatically. 
%Specifically, we will apply double-buffering automatically on all the on-chip buffers inside the I/O modules, and choose the maximal feasible\footnote{Data-packing factors should be divisors of the last dimension of the packed array and do not surpass the maximal packable elements threshold set by the compiler. By default, we set the data-packing factors upper bound in AutoSA using the argument \texttt{kernel[]->data\_pack[8,64,64]}. With this argument, we instruct AutoSA to pack at most 8/64/64 bytes of data between L1/L2/L3 I/O modules.} data-packing factors for maximizing the on-chip data transfer throughput. In the future, we will consider extending the framework to consider the tuning options in the communication management, such as the selection of double buffering and data packing factors.
Table~\ref{table:odyssey_design_space} summarizes the design space covered by Odyssey. Odyssey explores different dataflows in the space-time transformation and the loop tiling factors in array partitioning, latency hiding, and SIMD vectorization. Odyssey also explores non-divisor tiling factors and loop permutation in the step of array partitioning. When a non-divisor tiling factor is chosen, the original problem dimension is zero padded to be a multiple of the tiling factor. 
%Otherwise, additional loop guards are inserted that introduce unnecessary hardware overheads.
Tiling factors of latency hiding and SIMD vectorization are still required to be divisors as the array dimension is fixed after array partitioning and non-divisor tiling factors at later steps introduce prologue/epilogue phases and costly max/min operations that hurt the design performance. 
%If a non-divisor tiling factor is found by the auto-tuner, we ask the programmer to manually modify the original problem dimension to be a multiple of the tiling factor. Otherwise, additional loop guards will be inserted in the HLS program that lead to inferior performance.
%Tiling factors of latency hiding and SIMD vectorization are required to be divisors as the sub-array dimension is fixed after the array partitioning and non-divisor tiling factors will introduce prologue/epilogue phases in the computation and costly max/min operations in the generated hardware. 
%Lastly, Odyssey explores loop permutation in the step of array partitioning. As will be explained later, different loop orderings in the array partitioning band may lead to different performance.

\subsection{Supported Applications}
We limit the input programs to ones with rectangular iteration domains. The current framework cannot generate performance models automatically for programs with non-rectangular iteration domains such as LU decomposition. For such a case, programmers may implement the design performance models in Python files manually and supply it to the auto-tuner.
